Shortest Path to Boundary for Self-Intersecting Meshes

We introduce a method for efficiently computing the exact shortest path to the boundary of a mesh from a given internal point in the presence of self-intersections. We provide a formal definition of shortest boundary paths for self-intersecting objects and present a robust algorithm for computing the actual shortest boundary path. The resulting method offers an effective solution for collision and self-collision handling while simulating deformable volumetric objects, using fast simulation techniques that provide no guarantees on collision resolution. Our evaluation includes complex self-collision scenarios with a large number of active contacts, showing that our method can successfully handle them by introducing a relatively minor computational overhead.

==> Depr3cated_05_Implementation.tex <==
\section{Implementation}
\label{sec:Implementation and Acceleration}

\subsection{Shortest Path Query}
We use the open-source BVH implementation of \cite{wald2014embree} for both collision detection and closest point query.
We construct a scene including the tetrahedra from all meshes for collision detection and a separate scene for each mesh's surface for the shortest path query (\autoref{alg:ShortestPathToSurface}).

We have two implementations for each tetrahedral traverse algorithm: the static version and the dynamic version.
In the static version of the implementation, the candidate intersecting face stack $F$, the candidate next tetrahedron stack $T$, and the traversed tetrahedra list $\mathcal{T}$ are all aligned static array  on stack memory, which best utilizes the cache and SMID instructions of the processor. 
Of course, the static version of the algorithm will fail when the members in those arrays have exceeded their capacity. In those cases, the dynamic version will act as a fail-safe mechanism. The dynamic version of the traverse algorithm supports dynamic memory allocation thus those arrays can change size on the runtime. By carefully choosing the size of those static arrays, we can make sure most of the tetrahedral traverse is handled by the static implementation, optimizing efficiency and memory usage.

We also add some acceleration tricks to the implementations. First, we find that all the infinite loops encountered by the tetrahedral traverse only contain a few tetrahedra. Actually, the size of the loop is unbounded by the max number of tetrahedra adjacent to a vertex/edge. In practice, the number is even much smaller than that. Thus it is unnecessary to keep all the traversed tetrahedra in an array and check them at every step for the loop. Instead, we only keep the newest 16 traversed tetrahedra. In all our experiments, we have never encountered a loop with a size larger than 16.
$\mathcal{T}$ is implemented as a circular array and the oldest member will be automatically overwritten by the newest member. The array of size 16 can be efficiently examined by the SMID instructions. This modification significantly reduced the memory consumption and the running time of our method.

For the parameters of the algorithm, we $\epsilon_r = 0.01$.  $\epsilon_i$ is related to the scale and unit of the object, when the unit is the meter and the object is at a scale of a few meters, we set $\epsilon_i=1^{-10}$. We set the size of the static arrays in the static tetrahedral traverse algorithm to 32.
\subsubsection{Parallelism}
We would like to point out that the shortest path query for each penetrated point is embarrassingly parallel because the process can be done completely independently. All the querying threads will share the BVH structure of the surface and the topological structure of the tetrahedral mesh. During the execution no modification to those data is needed, thus no communication is needed between those threads. Also, our shortest path querying algorithm, especially the version with static arrays, can be efficiently executed on GPU.
\subsubsection{Overhead}
In contrast to SDF-based methods, the overhead of our method is very low. We only need to update the BVH structure for each mesh after the mesh has been deformed, which is the only overhead of our algorithm. Updating the bounding boxes of BVH is parallel and can be done with time complexity of $O(n)$, where $n$ is the number of surface primitives. This is very low in comparison to the update of an SDF.
In the use case of collision handling, the number of penetrated points is generally very small. As a result, it is the efficiency of overhead computation rather than the efficiency of the querying that determines the total running time.
As shown in \ref{sec:results}, our querying algorithm only takes less than $\%5$ of the total running time.

\subsection{Collision Handling}
We implement two types of DCD: vertex-tetrahedron collision detection and edge-tetrahedron collision detection. After detecting collisions, we query the shortest path right away. For edge-tetrahedron collision, we only query the shortest path for the point at the center of the edge-tetrahedron intersection. If there are more than one tetrahedra intersecting with the edge, we choose the one that is closest to the center of the edge. The idea is by keep pushing the center of the edge-tetrahedron intersection out, it will eventually resolve the whole intersection.

We model the collision constraint with the method of PBD\cite{muller2007position} or Projective Dynamics\cite{bouaziz2014projective}, i.e., by defining a collision plane at the closest point on the boundary $\mathbf{s}$ and the surface normal $\mathbf{n}$ at $\mathbf{s}$.
The constraint will project the penetrated point to the other (outer) side of the plane. Note that $\mathbf{s}$ locates on the edge or vertex, we use the smoothed normal instead of face normal to avoid discrepancy of normal computed from the different face. The friction was implemented as suggested by \cite{bender2015position}.

\subsection{Simulation  Framework}
We use XPBD as our simulation framework to solve the material and collision constraints. We use either mass-spring or NeoHookean \cite{macklin2021constraint} material to simulate the deformable body. 
In addition to DCD, we also implement CCD and build them into our simulation framework. CCD makes our framework insensitive to the time step. However, XPBD cannot guarantee to resolve all the collisions, thus relying solely on CCD will cause the simulation to fail eventually.
Thus at the beginning of each time step, we do an initial collision detection to separate the surface elements into two groups: already penetrated ones and penetration-free ones. Then after each XPBD step, we do CCD for those initially penetration-free ones and do DCD for those already penetrated ones. We find this hybrid system to be  very efficient and robust at the same time, combining the advantages of both CCD and DCD.

As suggested by \citet{macklin2016xpbd}, we trade substeps for iterations in the simulation framework. Within each substep, we do a small and constant number of 3 iterations to stabilize the collision solving. In each substep, we update the BVH and build collision constraints once and retain those constraints for subsequent iterations.


We choose a simple simulation framework (XPBD) to demonstrate the power of the exact penetration depth and the shortest path to the surface that our method provides.
If powered by our algorithm, even a straightforward framework like XPBD can produce those challenging or even unprecedented demos displayed in the following sections.






==> Deprecated_03_ShortestPathToBoundary_old.tex <==
\section{Shortest Path to Surface}
Resolving collided meshes is relatively easy when there is no self-intersection. For example, if we have one mesh intersecting another, we can resolve the collision by moving one's penetrating elements along the shortest path to the surface of the other mesh. The length of that shortest path is also called penetration depth \cite{van2003collision}, and response forces or constraints can be computed based on that depth to push collided meshes away. 

However, things become much more complicated when models can have arbitrary self-intersections. This is because the penetration depth for a surface point on the self-intersecting part of a mesh is not well defined. A penetrating surface point's Euclidean closest point on the surface is itself. However, this information will not help resolve the collision. In this case, the surface point is actually intersecting with an internal point of the mesh. Their positions overlap geometrically, but topologically they are different points. In fact, to fix the self-intersection, we have to move the penetrated surface point along its overlapping internal point's shortest path to the surface. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/01_GlobalGeoDesicPath.pdf}
    \caption{(a) In a mesh $M$ with self-intersection, a surface point $\mathbf{s}\in\partial{M}$ has penetrated $M$ and overlaps with an interior point $\mathbf{p}\in M$. The blue line illustrates the global geodesic path connecting $\mathbf{s}$ and $\mathbf{p}$. (b) Zoom in to the location of $\mathbf{s}$ and $\mathbf{p}$, where $\mathbf{s}$ locates in the surface of $M$, and $\mathbf{s}$ locates in the interior of another side of the $M$, where the intersection happens. (c) $\mathbf{p}$'s actual global geodesic path to $\partial{M}$, and its geodesic closest point on the surfaces: $\mathbf{s}'$.}
    \label{fig:GlobalGeoDesicPath}
\end{figure}
To better formulate the question, we introduce some notations. Say we have a $N$ dimensional manifold $M$, which is either a 2D mesh immersed in 2D space or a 3D mesh immersed in 3D space. $\partial{M}$ being $M$'s surface, which is a $(N-1)$D manifold. For a surface point $\mathbf{s}\in \partial{M}$, if it intersects with $M$, then, it must be overlapping with an $M$'s internal point $\mathbf{p}$, see Fig.\ref{fig:GlobalGeoDesicPath}(b). Note that there can be multiple $\mathbf{p}$, when there are multiple self-penetrations. Without loss of generality, we assume $\mathbf{s}$ only intersects with one interior point of $M$.
To resolve this self-intersection, we need to move $\mathbf{s}$ along its global geodesic path to $\partial{M}$ to resolve collision. Even though $\mathbf{s}$ locates on $\partial{M}$ and $|\mathbf{p}-\mathbf{s}|=0$, $\mathbf{p}$'s global geodesic path to $\partial{M}$, is not the geodesic path connecting $\mathbf{p}$ and $\mathbf{s}$, since the geodesic path can only pass through the interior of the model. As illustrated by Fig.\ref{fig:GlobalGeoDesicPath}a, the actual global geodesic path connecting $\mathbf{p}$ and $\mathbf{s}$, need to take a detour and is actually quite long. Though $\mathbf{p}$'s global geodesic path to an arbitrary point on the $\partial{M}$ is complicated, the case of $\mathbf{p}'s$ actual shortest path to the surface is much simpler.
We note an interior point $\mathbf{p}$'s global geodesic path to $\partial{M}$ as $l(p)$. Then $l_s(p)$ must satisfy the following properties:
\begin{itemize}
    \item $l_s(p)$ must be a straight line segment.
    \item $l_s(p)$ must be embedded in $M$.
    % \item For every point on $l(p)$ its global geodesic path to $\partial{M}$ is a subset of $l(p)$.
\end{itemize}

%The proof of those properties are trivial. Here we prove a brief proof of the first property. 
From the first property, we can sentence that, if a global the geodesic path be between an interior point $\mathbf{p}$ and a surface point $\mathbf{s}\in \partial{M}$ is not a straight line, that path is not $\mathbf{p}$'s shortest path to surface. 
The second property filters out the case like the zero-length line segment connecting $\mathbf{p}$ and $\mathbf{s}$ in Fig.\ref{fig:GlobalGeoDesicPath}a, and the line segment connecting $\mathbf{a}$ and $\mathbf{b}$ in Fig.\ref{fig:GlobalGeoDesicPath}c. 
Note that in the following sections when we mention a point on $M$, we refer to not only its position in the immersion space but also the actual embedding of that point,  to avoid ambiguity in the self-overlapping region. We note the line segment connecting $\mathbf{a}$ and $\mathbf{b}$ as $l(\mathbf{a}, \mathbf{b} )$.
Though line segment $l(\mathbf{a}, \mathbf{b} )$ is completely contained in $M$ in the immersion space, it is not embedded in $M$. Because $l(\mathbf{a}, \mathbf{b} )$ is not topologically continuous inside $M$. When moving from $\mathbf{a}$ to $\mathbf{b}$, the line will get out from the boundary of $M$, and connects to an interior point on another side of the mesh. This interior point, does not topologically connect to the boundary point it just passes through, thus $l(\mathbf{a}, \mathbf{b} )$ is not embedded in $M$. 

To simplify the notification, in the following sections, we will mainly discuss our to the case of 3D meshes immersed in 3D space, i.e., the case of tetrahedral meshes. However, the algorithm and notions we talk about can be trivially extended to the case of 2D meshes immersed in 2D space. 
For tetrahedral meshes, we propose the notion of \textit{tetrahedral traverse}, to provide a convenient way to determine whether a line is embedded in the mesh $M$:
\begin{definition}[Tetrahedral Traverse]
For a tetrahedral mesh $M$, and two point $\mathbf{a}, \mathbf{b}\in M$, a line segment is a valid tetrahedral traverse, if, there exists a list of tetrahedra $\mathcal{T} = (t_1, t_2, t_3, \dots, t_k)\subset M$, where $\mathbf{a}\in t_1$, $\mathbf{b}\in t_k $, and $t_i$ and $t_{i+1}$ is topologically connected for  $1 \leq i \leq k-1$, i.e., they share a common face, edge or vertex.
\end{definition}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/02_TetrahedralTraverse.pdf}
    \caption{(a) An example of a triangular traverse, marked by red triangles. A line segment connecting $\mathbf{a}$ and $\mathbf{b}$ is embedded in this triangular traverse.  (b) An example of a line segment cannot be embedded in a manifold when there are self-intersections, the triangular traverse (marked by the red triangles) stops at the boundary of the mesh but the line segment penetrates the boundary an continue going. In this case the line cannot be embedded into $M$. }
    \label{fig:TetrahedraTraverse}
\end{figure}
Similarly, we can define \textit{triangular traverse} for the case of 2D meshes immersed in 2D space. 

In other words, a tetrahedral traverse is a sequence of topologically connected tetrahedra from a tetrahedral mesh. It can be easily seen that a line segment can be embedded in the tetrahedral mesh, if and only if it can be embedded in a tetrahedral traverse $\mathcal{T} \subset M$, see Fig.\ref{fig:TetrahedraTraverse}. 
Then we can determine whether a line segment is embedded in $M$ by trying to construct a tetrahedral/triangular traverse. We say a line segment $l$ is a \textit{valid tetrahedral traverse of $M$}, if $l$ can be embedded in a tetrahedral traverse $\mathcal{T}\subset M$.




\begin{algorithm}[t]
\SetAlgoNoLine
\KwIn{A surface point $\mathbf{s} \in M$, a target internal point $\mathbf{p}$, half face $t_0$ containing $\mathbf{s}$. }
\KwOut{Boolen value representing whether there is a valid tetrahedral traverse between $\mathbf{s}$ and $\mathbf{p}$.}
$T=\{t_0\}$, $C=\emptyset$ \;
$\mathbf{d}=\frac{\mathbf{t}-\mathbf{p}}{\|\mathbf{t}-\mathbf{p}\|}$\;
\While{$T\neq \emptyset$}{
    pick $t\in T$, $T = T \setminus \{t\} $\;
    $c$ = the tetrahedron that $t$ belongs to\;
    \eIf{$c \in C$}{
        continue;
    }{
        $C=C\cup \{c\}$
    }
    \If{$p \in c$}{
        return True\;
    }
    
    \For { each half face $t' \in$ all $c$'s half faces}{
        \If{$t=t'$}{continue\;}
        \If{LineTriangleIntersection($\mathbf{s}, \mathbf{d}, t'$)}{
            \eIf{$t'$ is surface triangle}{
                return False;
            }{
                $t'' = $ the dual half face of $t'$\;
                $T=T\cup \{t''\}$\;
            }
        }    
    }
    
}
\caption{TetrahedralTraverse}
\label{alg:one}
\end{algorithm}
